Radiation Damage Study for PHENIX Silicon Stripixel Sensors

Silicon stripixel sensors which were developed at BNL will be installed as part of the RHIC-PHENIX silicon vertex tracker (VTX). RHIC II operations provide luminosity up to 2x10^32 /cm2/s so the silicon stripixel sensors will be exposed to a significant amount of radiation. The most problematic radiation effect for VTX is the increase of leakage current, which degrades the signal to noise ratio and may saturate the readout electronics. We studied the radiation damage using the same diodes as CERN-RD48. First, the proportionality between the irradiation fluence and the increase of leakage current of CERN-RD48 was reproduced. Then beam experiments with stripixel sensor were done in which leakage current was found to increase in the same way as that of thereference diode. A stripixel sensor was also irradiated at the PHENIX interaction region (IR) during the 2006 run. We found the same relation between the integrated luminosity and determined fluence from increase of leakage current. The expected fluence is 3-6x10^12 Neq/cm2 (1 MeV neutron equivalent) in RHIC II operations for 10 years. Due to this expected exposure, setting the operating temperature in PHENIX to T< 0 deg. C to suppress leakage current is needed to avoid saturation of preamplifiers.

==> Makefile <==
NIMmain.pdf: NIMmain.tex \
	author.tex \
	abstract.tex \
	introduction.tex \
	stripixel.tex \
	rad-damage.tex \
	IRtest.tex \
	beamtest.tex \
	conclusion.tex \
	reference.tex \
	beam-stripixel.tex

	latex NIMmain.tex
	latex NIMmain.tex
	dvipdf NIMmain
 

